Deep learning meets tree phenology modeling: PhenoFormer vs. process-based models

Phenology, the timing of cyclical plant life events such as leaf emergence and coloration, is crucial in the bio-climatic system. Climate change drives shifts in these phenological events, impacting ecosystems and the climate itself. Accurate phenology models are essential to predict the occurrence of these phases under changing climatic conditions. Existing methods include hypothesis-driven process models and data-driven statistical approaches. Process models account for dormancy stages and various phenology drivers, while statistical models typically rely on linear or traditional machine learning techniques. Research shows that process models often outperform statistical methods when predicting under climate conditions outside historical ranges, especially with climate change scenarios. However, deep learning approaches remain underexplored in climate phenology modeling. We introduce PhenoFormer, a neural architecture better suited than traditional statistical methods at predicting phenology under shift in climate data distribution, while also bringing significant improvements or performing on par to the best performing process-based models. Our numerical experiments on a 70-year dataset of 70,000 phenological observations from 9 woody species in Switzerland show that PhenoFormer outperforms traditional machine learning methods by an average of 13% R2 and 1.1 days RMSE for spring phenology, and 11% R2 and 0.7 days RMSE for autumn phenology, while matching or exceeding the best process-based models. Our results demonstrate that deep learning has the potential to be a valuable methodological tool for accurate climate-phenology prediction, and our PhenoFormer is a first promising step in improving phenological predictions before a complete understanding of the underlying physiological mechanisms is available.

==> 6_coverpage.tex <==
\section*{Deep learning meets tree phenology modeling: PhenoFormer vs. process-based models}


\textbf{AUTHORS:}

 Vivien Sainte Fare Garnot $^1$,  Lynsay Spafford $^{2,3}$,  Jelle Lever,  $^3$ Christian Sigg $^4$,  Barbara Pietragalla $^4$,  Yann Vitasse $^3$,  Arthur Gessler $^3$,  Jan Dirk Wegner $^1$


 $1$ : Department of Mathematical Modeling and Machine Learning (DM3L), University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland

$2$ : St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada 

$3$ : Swiss Federal Institute for Forest, Snow and Landscape Research (WSL), Zürcherstrasse 111, 8903  Birmensdorf, Switzerland

$4$ : Swiss Federal Office of Meteorology and Climatology (MeteoSwiss) Operation Center 1, 8058 Zürich-Flughafen, Switzerland


\textbf{CORRESPONDING AUTHOR:} Vivien Sainte Fare Garnot

Address: Department of Mathematical Modeling and Machine Learning (DM3L), University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland; E-mail: vivienyannisathanassios.saintefaregarnot@uzh.ch 


\textbf{RUNNING HEADLINE:} PhenoFormer: Deep learning for tree phenology modeling

\textbf{DATA AVAILABILITY:} All the data used in the present study will be made publicly available on Zenodo upon publication.

\textbf{AUTHOR CONTRIBUTIONS:}  Vivien Sainte Fare Garnot conceptualised the study, developed the deep learning methodology, ran the learning-based experiments, wrote the associated code, performed the formal analysis of the results, prepared the visualisations, and wrote the first version of the paper, Lynsay Spafford ran all the process-models experiments , wrote the associated code, and helped in the formal analysis and the drafting of the first version of the paper. Jelle Lever contributed to the formal analysis and to the reviwing and editing of the manuscript.
Barbara Pietragalla and Chrisitian Sigg helped in the curation of the phenological data used in the present study. Barbara Pietragalla, Chrisitian Sigg, Yann Vitasse, Arthur Gessler, and Jan Wegner helped in the formal analysis and the editing of the manuscript. Arthur Gessler and Jan Wegner secured funding for the research.



\textbf{The authors declare no conflicts of interest}

